Sparsity in Deep Neural Networks - An Empirical Investigation with TensorQuant

Deep learning is finding its way into the embedded world with applications such as autonomous driving, smart sensors and aug- mented reality. However, the computation of deep neural networks is demanding in energy, compute power and memory. Various approaches have been investigated to reduce the necessary resources, one of which is to leverage the sparsity occurring in deep neural networks due to the high levels of redundancy in the network parameters. It has been shown that sparsity can be promoted specifically and the achieved sparsity can be very high. But in many cases the methods are evaluated on rather small topologies. It is not clear if the results transfer onto deeper topologies. In this paper, the TensorQuant toolbox has been extended to offer a platform to investigate sparsity, especially in deeper models. Several practical relevant topologies for varying classification problem sizes are investigated to show the differences in sparsity for activations, weights and gradients.

==> text/INFO.tex <==


\section{First Section}
\subsection{A Subsection Sample}
Please note that the first paragraph of a section or subsection is
not indented. The first paragraph that follows a table, figure,
equation etc. does not need an indent, either.

Subsequent paragraphs, however, are indented.

\subsubsection{Sample Heading (Third Level)} Only two levels of
headings should be numbered. Lower level headings remain unnumbered;
they are formatted as run-in headings.

\paragraph{Sample Heading (Fourth Level)}
The contribution should contain no more than four levels of
headings. Table~\ref{tab1} gives a summary of all heading levels.

\begin{table}
\caption{Table captions should be placed above the
tables.}\label{tab1}
\begin{tabular}{|l|l|l|}
\hline
Heading level &  Example & Font size and style\\
\hline
Title (centered) &  {\Large\bfseries Lecture Notes} & 14 point, bold\\
1st-level heading &  {\large\bfseries 1 Introduction} & 12 point, bold\\
2nd-level heading & {\bfseries 2.1 Printing Area} & 10 point, bold\\
3rd-level heading & {\bfseries Run-in Heading in Bold.} Text follows & 10 point, bold\\
4th-level heading & {\itshape Lowest Level Heading.} Text follows & 10 point, italic\\
\hline
\end{tabular}
\end{table}


\noindent Displayed equations are centered and set on a separate
line.
\begin{equation}
x + y = z
\end{equation}
Please try to avoid rasterized images for line-art diagrams and
schemas. Whenever possible, use vector graphics instead (see
Fig.~\ref{fig1}).

\begin{figure}
%\includegraphics[width=\textwidth]{fig1.eps}
\includegraphics[width=\textwidth]{figures/test}
\caption{A figure caption is always placed below the illustration.
Please note that short captions are centered, while long ones are
justified by the macro package automatically.} \label{fig1}
\end{figure}

\begin{theorem}
This is a sample theorem. The run-in heading is set in bold, while
the following text appears in italics. Definitions, lemmas,
propositions, and corollaries are styled the same way.
\end{theorem}
%
% the environments 'definition', 'lemma', 'proposition', 'corollary',
% 'remark', and 'example' are defined in the LLNCS documentclass as well.
%
\begin{proof}
Proofs, examples, and remarks have the initial word in italics,
while the following text appears in normal font.
\end{proof}
For citations of references, we prefer the use of square brackets
and consecutive numbers. Citations using labels or the author/year
convention are also acceptable. The following bibliography provides
a sample reference list with entries for journal
articles~\cite{ref_article1}, an LNCS chapter~\cite{ref_lncs1}, a
book~\cite{ref_book1}, proceedings without editors~\cite{ref_proc1},
and a homepage~\cite{ref_url1}. Multiple citations are grouped
\cite{ref_article1,ref_lncs1,ref_book1},
\cite{ref_article1,ref_book1,ref_proc1,ref_url1}.

==> text/related_work.tex <==
\section{Related Work}

%% Very Relevant

%% Characterizing Sparse Connectivity Patterns in Neural Networks:
% Experiments on Sparsity \cite{dey2017characterizing}

%% Learning Structured Sparsity in Deep Neural Networks:
% Structured Sparsity is good for (GPU) performance. Layerwise Sparsity for AlexNet and L1. \cite{WenWu2016Learning}

%% EFFICIENT SPARSE-WINOGRAD CONVOLUTIONAL NEURAL NETWORKS:
% Combining Winograd with sparsity. Shows ResNet14 on ImageNet sparsity for weights and activations! \cite{LiuPoo2018Efficient}

%% Compressing DMA Engine: Leveraging Activation Sparsity for Training Deep Neural Networks:
% GPU DMA engine for less memory transfers in deep learning. Activations are sparse. Activation density during training in AlexNet! \cite{rhu2018compressing}

%% meProp: Sparsified Back Propagation for Accelerated Deep Learning with Reduced Overfitting:
% 99\,\% gradient sparsity without increase in iteration steps. Using top-k elements instead of threshold. Onlyresults for MLP with MNIST. \cite{SunRen17meProp}





%The most crucial operation in deep learning is the matrix-vector multiplication. The sparse variant of this increases efficiency a lot. Thankfully, a lot of work has been done in this field, appart from deep learning \cite{DorRen14Scalable, BelGar09Implementing}. This allows to transfer a lot of knowledge.


%% Architecture

%% SparseNN: An Energy-Efficient Neural Network Accelerator Exploiting Input and Output Sparsity: 
%Hardware architecture and FPGA implementation of accelerator which computes MV-products given as sparse. Layerwise quantization for LeNet and AlexNet. \cite{ZhuJia2017SparseNN}

%% SPARSELY-CONNECTED NEURAL NETWORKS: TOWARDS EFFICIENT VLSI IMPLEMENTATION OF DEEP NEURAL NETWORKS:
%Sparse MLP architecture, uses some dropout-like technique. Also a HDL architecture. \cite{ardakani2016sparsely}


%% EIE: Efficient Inference Engine on Compressed Deep Neural Network:
%Sparse Matrix DNN accelerator ASIC. \cite{HanLiu16EIE}

%% ACCELERATING DEEP CONVOLUTIONAL NETWORKS USING LOW-PRECISION AND SPARSITY:
% Ternary-gradients and zero-skipping in hardware accelerator desing. \cite{venkatesh2016accelerating}

%% A Novel Zero Weight/Activation-Aware Hardware Architecture of Convolutional Neural Network:
% Hardware Architecture for zero-skipping activations and weights. Showing sparstiy for pruned AlexNet. \cite{kim2017novel}

%% Cambricon-X: An Accelerator for Sparse Neural Networks:
% Hardware architecture which can cope with pruned sparse neural networks. \cite{zhang2016cambricon}

%% NullHop: A Flexible Convolutional Neural Network Accelerator Based on Sparse Representations of Feature Maps:
% Embedded System (FPGA) for DL image recognition, sparse feature maps. \cite{aimar2017nullhop}




%% Sparsity in Topology, while learning
%% LOG-DENSENET: HOW TO SPARSIFY A DENSENET:
% Remove skip connections in denseNet like topologies \cite{HuDey2017LogDenseNet}

%% DEEP DOUBLE SPARSITY ENCODER: LEARNING TO SPARSIFY NOT ONLY FEATURES BUT ALSO PARAMETERS:
% Learning Sparsity in encoder.\cite{WanHua2016Deep}

%% THE POWER OF SPARSITY IN CONVOLUTIONAL NEURAL NETWORKS
% Depth multiplier(layer width), random sparsity and incremental training. \cite{ChaSan2017Power}

%% DEEP REWIRING: TRAINING VERY SPARSE DEEP NETWORKS
% Rewiring, incremental learning \cite{bellec2017rewiring}

%% RE-WEIGHTED LEARNING FOR SPARSIFYING DEEP NEURAL NETWORKS:
% directly learn sparsity with affine scaling transformations. \cite{fedorov2018reweighted}

%% Sparse Convolutional Neural Networks:
% Reducing sparsity with sparse decomposition\cite{LiuWan2015Sparse}

%% ATTENTION-BASED GUIDED STRUCTURED SPARSITY OF DEEP NEURAL NETWORKS:
% Using group lasso to promote sparsity. Sparsity levels of 90\% in LeNet. Very precise regarding sources for topologies (get citations for them here) \cite{TorShi2018Attention}

%% Optimal brain damage:
% Removal of connections with help of second order information. \cite{CunDen90Optimal}

%% DEEP COMPRESSION: COMPRESSING DEEP NEURAL NETWORKS WITH PRUNING, TRAINED QUANTIZATION AND HUFFMAN CODING:
% Pruning reduces the network size by a factor of 35. Work on AlexNet and VGG16. \cite{HanMao16Deep}

%% EFFICIENT SPARSE-WINOGRAD CONVOLUTIONAL NEURAL NETWORKS:
%Combining Winograd with sparsity. Shows ResNet14 on ImageNet sparsity for weights and activations! \cite{LiuPoo2018Efficient}





%% Sparsity in Distributed Systems

%% SparCML: High-Performance Sparse Communication for Machine Learning:
% Communication Protocols for sparse data for distributed systems \cite{renggli2018sparcml}

%% Sparse Communication for Distributed Gradient Descent:
% Exchanging Sparse Matrices, using 1-bit quantization. On MNIST. \cite{AjiFik2017Sparse}

%% Compressing DMA Engine: Leveraging Activation Sparsity for Training Deep Neural Networks:
% GPU DMA engine for less memory transfers in deep learning. Activations are sparse. Activation density during training in AlexNet! \cite{rhu2018compressing}

%% Gradient Sparsification for Communication-Efficient Distributed Optimization:
% Randomly dropout gradient coordinates and amplify others. Reduces communication costs during training \cite{WanWan2018Gradient}




%% Theory
%% Optimal Approximation with Sparsely Connected Deep Neural Networks:
% Theoretical boundaries for connectivity and memory 

%% Non-DL Sparsity
%% A Scalable Sparse Matrix-vector Multiplication Kernel for Energy-efficient Sparse-blas on FPGAs:
% Sparse Kernel on FPGA \cite{DorRen14Scalable}

%% Implementing Sparse Matrix-vector Multiplication on Throughput-oriented Processors:
% Sparse MV-Multiplication on GPUs. \cite{BelGar09Implementing}
